Dimension-reduced KRnet maps for high-dimensional Bayesian inverse problems

We present a dimension-reduced KRnet map approach (DR-KRnet) for high-dimensional Bayesian inverse problems, which is based on an explicit construction of a map that pushes forward the prior measure to the posterior measure in the latent space. Our approach consists of two main components: data-driven VAE prior and density approximation of the posterior of the latent variable. In reality, it may not be trivial to initialize a prior distribution that is consistent with available prior data; in other words, the complex prior information is often beyond simple hand-crafted priors. We employ variational autoencoder (VAE) to approximate the underlying distribution of the prior dataset, which is achieved through a latent variable and a decoder. Using the decoder provided by the VAE prior, we reformulate the problem in a low-dimensional latent space. In particular, we seek an invertible transport map given by KRnet to approximate the posterior distribution of the latent variable. Moreover, an efficient physics-constrained surrogate model without any labeled data is constructed to reduce the computational cost of solving both forward and adjoint problems involved in likelihood computation. With numerical experiments, we demonstrate the accuracy and efficiency of DR-KRnet for high-dimensional Bayesian inverse problems.

==> krnet.tex <==
The basic idea of KRnet is to define the structure of $f({x})$ in terms of the Knothe-Rosenblatt rearrangement. Let $\mu_Z$ and $\mu_X$ be the probability measures of two random variables $X,Z\in\xs{R}^d$ respectively. A mapping $\mathcal{T}$: $Z \mapsto X$ is called a transport map such that $\mathcal{T}_{\#} \mu_Z = \mu_X$, where $\mathcal{T}_{\#} \mu_{Z}$ is the push-forward of $\mu_{Z}$ such that $\mu_{X}(B) = \mu_{Z}(\mathcal{T}^{-1}(B))$ for every Borel set $B$. The Knothe-Rosenblatt rearrangement tells us that the transport map $\mathcal{T}$ may have a lower-triangular structure 
\begin{equation}
    {z} = \mathcal{T}^{-1}({x}) = \left[ 
    \begin{array}{l}
    \mathcal{T}_1(x_1) \\
    \mathcal{T}_2(x_1, x_2) \\
    \vdots \\
    \mathcal{T}_{d}(x_1, \ldots, x_d)
    \end{array}
    \right].
\end{equation}
This mapping can be regarded as a limit of sequence of optimal transport maps when the quadratic cost degenerates \cite{carlier2010knothe}. Noticing that the invertible mapping $f(x)$ also defines a transport map, we then incorporate the triangular structure of the Knothe-Rosenblatt rearrangement into the definition of $f(x)$ which results in KRnet as a generalization of real NVP \cite{dinh2016density}. Let ${x} = [{x}^{(1)}, \ldots, {x}^{(K)}]^\mathsf{T}$ be a partition of ${x}$, where ${x}^{(i)} = [x_{1}^{(i)}, \ldots, x_{m}^{(i)}]^\mathsf{T}$ with $1 \leq K \leq d, 1 \leq m \leq d$, and $\sum_{i=1}^K \mathrm{dim}({x}^{(i)}) = d$. Our KRnet takes an overall form
\begin{equation} \label{eqn_KR}
  {z} = f({x}) = \left[ 
    \begin{array}{l}
    f_1({x}^{(1)}) \\
    f_2({x}^{(1)}, {x}^{(2)}) \\
    \vdots \\
    f_{K}({x}^{(1)}, \ldots, {x}^{(K)})
    \end{array}
    \right].
\end{equation}
Here each $f_{i}$ is an invertible mapping  for $ i = 2, \ldots, K$. Each $f_{i}$ is constructed by stacking a sequence of simple bijections, each of which is a shallow neural network, and thus the overall mapping $f$ is a deep neural network. KRnet consists of one  outer loop and $K-1$ inner loops. The outer loop has $K-1$ stages, corresponding to the $K-1$ mappings $f_{i}$ in equation \eqref{eqn_KR} with $i=2,\ldots,K$, and for each stage, an inner loop of $L$ affine coupling layers is defined. More specifically, we have
\begin{equation}\label{krnet_expr}
z = f(x) = L_{N} \circ f_{[K-1]}^{\textsf{outer}} \circ \cdots \circ f_{[1]}^{\textsf{outer}} (x),
\end{equation}
where $f_{[i]}^{\textsf{outer}}$ is defined as
\begin{equation}
f_{[k]}^{\textsf{outer}} = L_S \circ f_{[k, L]}^{\textsf{inner}} \circ \cdots \circ f_{[k,1]}^{\textsf{inner}} \circ L_R.
\end{equation}
Here $f_{[k,i]}^{\textsf{inner}}$ indicates a combination of one affine coupling layer and one scale and bias layer, and $L_N$, $L_S$ and $L_R$ indicate the nonlinear layer, the squeezing layer and the rotation layer, respectively.
More details about KRnet can be found in \cite{tang2020deep,adda_2022}.

